Object-centric Forward Modeling for Model Predictive Control

We present an approach to learn an object-centric forward model, and show that this allows us to plan for sequences of actions to achieve distant desired goals. We propose to model a scene as a collection of objects, each with an explicit spatial location and implicit visual feature, and learn to model the effects of actions using random interaction data. Our model allows capturing the robot-object and object-object interactions, and leads to more sample-efficient and accurate predictions. We show that this learned model can be leveraged to search for action sequences that lead to desired goal configurations, and that in conjunction with a learned correction module, this allows for robust closed loop execution. We present experiments both in simulation and the real world, and show that our approach improves over alternate implicit or pixel-space forward models. Please see our project page (https://judyye.github.io/ocmpc/) for result videos.

==> 1draft.tex <==
\href{https://docs.google.com/presentation/d/1ckPVxXHP5kKjBEBDCzIggIkc8gbVoQZZnsYTj5KrtGE/edit?usp=sharing}{Slides}
\subsection{Problem Setup}

\paragraph{Figuring out what problem to solve. } We answer some of these questions: 
\begin{enumerate}
    \item Does structure in prediction module help the control? 
    \item In what sense structure helps?  (Evaluation / what we want to achieve at last)
    \begin{enumerate}
        \item A better evaluation metric of action? 
        \item Clutter setting? 
        \item Generalization? Robust? Transfer across task? 
    \end{enumerate}
    \item What structure would be useful? or what information should structure encode? 
    \begin{enumerate}
        \item The structure should depends on action.
        \item Can structure encode constraints in action / state space? - gives us a cost map.
        \item Multiple object coupling? 
    \end{enumerate}
\end{enumerate}

